Strengthening SDN Security: Protocol Dialecting and Downgrade Attacks

Software-defined networking (SDN) has become a fundamental technology for data centers and 5G networks. In an SDN network, routing and traffic management decisions are made by a centralized controller and communicated to switches via a control channel. Transport Layer Security (TLS) has been proposed as its single security layer; however, use of TLS is optional and connections are still vulnerable to downgrade attacks. In this paper, we propose the strengthening of security assurance using a protocol dialecting approach to provide additional and customizable security. We consider and evaluate two dialecting approaches for OpenFlow protocol operation, adding per-message authentication to the SDN control channel that is independent of TLS and provides robustness against downgrade attacks in the optional case of TLS implementation. Furthermore, we measure the performance impact of using these dialecting primitives in a Mininet experiment. The results show a modest increase of communication latency of less than 22%.

==> Notes/limitations_removed.tex <==
\begin{comment}

While not implemented in this research, we anticipate that a policy enforcement proxy (PEP) could determine which key to use in a multi switch system through the assignment of port addresses for each proxy. We assume that one proxy would be paired with one end-device. Therefore, that proxy must contain a method to manage multiple connections. The ability to manage identities and keys can be linked by using assigned port numbers at the IP level without requiring management at the derivative level. Additional logic would require the registration of a new proxy for each device added to the system. This method is similar to the process of white-listing where each additional unit is registered at each policy enforcement proxy. 

We anticipate that the addition of a dialect to a system that is already in use could identify attackers on a network and provide additional security to virtual private network guests. For example, if derivatives are added one system at a time and verified then a network size and topography can be known. If a network has been created and is unknown in size or registration then only systems that are trusted can have policy enforcement proxies added to them. 


The addition of a policy enforcement proxy then provides a way of identifying network traffic that is authentic to the network. For instance, when attackers can attempt to hide within traffic they are actually attacking from outside a network. The derivative would not be included in the normal traffic and could then be investigated further or blocked. The addition of a derivative would then provide a method for identifying traffic that is not authentic and still on the network attempting to access other systems or data.

The dialect, only provided to critical systems, would identify attackers attempting to reach systems that they previously had access to. For example, the ability to filter systems that are accessible through a virtual private network can then be limited to only performing actions with a unit that is not speaking the dialect.  


The experimental policy enforcement proxy provides notification when a dialect security policy has been violated via the terminal. The proxy will then send a message to the controller and switch which terminates the connection. In the event that a network already has an IDS, notifications of policy violations can be passed to the IDS to provide additional security response and logging. Therefore, a dialect provides another means of log collection and analysis for real-time security. 


The flexibility of a policy enforcement proxy implemented as a proxy also allows for variable security mechanisms. Packet inspection allows for a variety of features, settings, data, and conditions to be met in order to allow the packet to continue to the protected end-device. For example, if an SDN system is not yet TLS capable, the installation of the proxies could add both TLS and the dialect. This scenario may also be similar to industrial control systems where physical security and obscurity is relied upon. The use of an all-in-one additional security pair can add security for different types of devices besides a controller and switch. 


An additional design choice for the use of proxies to provide security for downgrade attacks would be for the stateful inspection of the TLS Hello messages to force connections to be no lower than a specified TLS version. This would also be useful outside of the dialect design to prevent unwanted behavior from various switches and controllers.


Lastly, future work would include the design and implementation of a plug-and-play, all-in-one policy enforcement proxy. This proxy would have an interface for programming and network connections. This one device would perform all of the steps of the protocol dialect process and provide options to the network manager for implementation. This system could also provide other options for multi-factor authentication, nonce sharing that is out of bound, threaded for asymmetric communication, and able to perform communications with an unlimited number of other policy enforcement proxies. 


\end{comment}

==> Notes/seudo_code_backup.tex <==
\sout{For the purpose of rapid prototyping, we implemented the proxy functionality with Python.  A pseudo-code overview for the TCP connection management part of the controller proxy logic is provided below. %This overview provides for TCP connections between the proxies and their associated devices. 
Performance limitations associated with this generic communication style and the use of Python are described in Section~\ref{sec:discussion}.  The entire Python code is available online, via the same web link provided at the end of Section~\ref{sec:evaluation}. } 

\sout{\redtext{Dan: commented out sudo code}}


% % footnote size may be too small for formatting rules? (10 pt is the minimum
% {\small
% \begin{verbatim}
   
%     controller_sock = make_socket
%     controller_sock.connect
%     proxy_to_proxy_sock = make_socket
%     proxy_to_proxy_sock.listen(1)
   
%     ikm = hmac_sha512(KEY_OOB, SALT)
%     salt = get_salt()
%     key = hkdf(ikm)
   
%     data = proxy_connection.recv
%     receipt = D1_check(receipt, ikm, salt)
%     if(receipt == PASS):
%       D1_pass = True
%     else:
%       D1_pass = False
    
%     while(true):
%         data = proxy_connection.recv
%         receipt = D2_check(receipt, ikm, salt)
%         if(receipt == PASS):
%             controller_sock.sendall(receipt)
%         else:
%             controller_sock.sendall(FAIL_MSG)

%         data = controller_sock.recv()
%         receipt = D2_create(receipt, ikm, salt)
%         proxy_connection.sendall(receipt)
        
% \end{verbatim}
% }


==> Prior_to_Swap_files/analysis.tex <==
\section{Security Basis}
\label{sec:analysis}


In this section we consider the composite security of D1 and D3, based on the design choices discussed in Section~\ref{sec:method}.  

\subsection{Formalizing Design Choices}

Prior to implementation of D1 and D3, a symmetric key generated at random, is established out-of-band (OOB).\footnote{This may occur as an OOB key distribution. However, there is the potential to embed a full key exchange in a prior run of D2 or D3; we leave this as future work.} It is assumed that keys used between a controller and switch are not reused for any other controller/switch pair. Following the initial key distribution, each side generates uni-directional keys (UDK) for D1 and D3 according to Fig.~\ref{fig:keyderivation} and Fig.~\ref{fig:keyusage}, where $K_{ab}$ indicates the symmetric key used to protect data from $a$ to $b$ and $ || $ indicates concatenation.


\begin{figure}[htbp!]
    \centering
    \includegraphics[width=60mm]{figs/Key_Derivation.jpeg}
    \caption{D1, D3 Key Derivation. $KDF$ represents the key derivation function, $TS_a$ indicates the timestamp for party $a$, $K_{ab}$ indicates the symmetric key used uni-directionally between $a$ and $b$, and $sid$ represents the session identifier which we calculate as \mbox{$sid= D1\_MAC\_Switch||D1\_MAC\_Controller$}.}
    \label{fig:keyderivation}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=90mm]{figs/D1_D3_Process.jpeg}
    \caption{D1, D3 Key Usage. Horizontal flows indicate (potentially) non-interactive messages such that ordering is not enforced. Angled flows indicate interactive messages with enforced ordering. $SN_a$ indicates sequence number for party $a$, $TS_a$ indicates the timestamp for party $a$.}
    \label{fig:keyusage}
\end{figure}




The inclusion of a timestamp in the key derivation on each side constitutes a potential point of failure, and is dependent on the implementation method.  However, the timestamp could be computed based on the completion of the TCP handshake to limit clock de-synchronization.

Note that we use the transcript MAC values of the initial flows to provide continuity to the communication between D1 and D3, essentially employing these as a session identifier.  This links D1 protection to D3, follows other accepted protocol practice, such as in TLS, where a server and client commit to the transcript of handshake messages.

Initially, the proxies will exchange D1 messages (potentially) non-interactively.
The freshness value incorporated in our design is based on implicit timestamps using epoch time (rounded to seconds). This has implied assumptions that the controller and switch have the same clock time, which is reasonable with embedded hardware clocks. Packets arriving during the same second should pass MAC verification, while those arriving outside of the time window will fail verification.
Note that we do not employ such freshness values simply to inhibit replay attacks; the MAC length is limited in D1 by the 32-bits and as a result is liable to 2nd-preimage attacks. Consequently, it is necessary to limit the viable lifespan of the MAC, which is performed via the viability window.   
Any packet received outside of this window will have a different key used in the MAC calculation step.  Therefore, if an attacker attempted to replay any messages, then they must be replayed within the same time window in order to pass the MAC verification step.


\subsection{D1 Security}

The security goal of D1 is to establish that the proxies involved possess the correct keys, perform MAC verification, and establish a session identifier to be used for consistency in the D3 MAC verification stage. Thus D1 acts, in part, as a mutual authentication protocol with associated data. We reference \cite{rogaway2009authentication} for a technique for more in-depth computational analysis of such composed protocols with associated data. 
An attacker's goal of breaking entity authentication during D1 is largely dependent on breaking the security of the MAC. This again highlights the importance of limiting the MAC lifespan through validity windows, due to the relatively short MAC output length used during D1.

To assess the security of D1, we seek to conduct a comparison with a previously analyzed protocol.  The D1 process can be compared to the repaired ISO/IEC 9798-4:1999 Mechanism 5.2.1 two-pass mutual authentication protocol (referred to as ISO 9798-4-3 by Cremers et al.) \cite{basin2013provably,ISO9798}, as shown in Fig.~\ref{fig:9798_compare}. We note and align the following differences.

\paragraph{Check Function} ISO/IEC 9798-4:1999 Mechanism 5.2.1 specifies the use of a cryptographic check function, with reference to those given in ISO/IEC 9797. This includes our choice of a MAC algorithm. From this point on we will assume that the cryptographic check function is a MAC.     

\paragraph{Uni-Directional Keys (UDK)}\label{par:first}
Cremers et al. \cite{basin2013provably} incorporate identities into the check function to show direction of flows, hence avoiding reflection attacks due the single symmetric key. D1 embeds this in the derivation process of the UDKs.  Each key derivation contains identifiers for the sender and the receiver.  This prevents messages sent by the switch to be accepted by the switch, e.g. a reflection attack.  Furthermore, the control plane of an SDN limits communication from a switch only to the controller (switches will not communicate with other switches). 
When UDKs are used, such as described above, the identities are no longer a necessary input to the cryptographic check function~\cite{ISO9798}.  




\paragraph{Text Fields} $Text_x$ values in Fig.~\ref{fig:9798_compare} correspond to the OpenFlow Hello messages sent by D1. Unlike in the original ISO/IEC 9798-4:1999 Mechanism 5.2.1, we do not allow for variable selection of data for these fields: it is pre-determined. Consequently, we also avoid the associated potential protocol flow syntax errors \cite{basin2013provably}.  

\paragraph{Timestamps}
The repaired ISO/IEC 9798-4:1999 Mechanism 5.2.1 explicitly sends timestamps ($TS_x$) and uses them as inputs to the MAC.  D1 uses implicit timestamps in order to conform as closely as possible to the OpenFlow Hello standard. These are still input as normal into the function, but are not sent explicitly as the switch and controller have shared knowledge of them.  

\paragraph{Flow Ordering}
Additionally, the repaired protocol~\cite{basin2013provably} uses a flow tagging value to ensure messages are correctly interpreted according to their order in the protocol, e.g. ``$\mathtt{Flow1}$'' and ``$\mathtt{Flow2}$''. As D1 proxies enforce ordering, the protocol flow generated by the switch will always be interpreted as the first flow, while the protocol flow from the controller will be held to be the second.


\paragraph{Protocol Version Confirmation}\label{par:last} As in \cite{basin2013provably}, we explicitly send the authentication protocol version (``$\mathtt{9798-4-5.2.1}$'') used in D1. 

With consideration of the above points a)--f), we map D1 to the repaired ISO/IEC 9798-4:1999 Mechanism 5.2.1, which achieves mutual authentication of party $A$ and $B$ \cite{basin2013provably}. Thus, D1 acts as a mutual entity authentication protocol for the subsequent D3 derivative.

\begin{figure}[htbp]
\begin{subfigure}{.48\textwidth}
  \centering
    \includegraphics[width=88mm, trim=30 0 0 0]{figs/9798_flow.jpeg}
    \caption{Repaired ISO/IEC 9798-4-5.2.1.}
    \label{fig:repaired_flow}
\end{subfigure}%

\begin{subfigure}{.48\textwidth}
  \centering
    \includegraphics[width=88mm, trim=0 0 25 0]{figs/D1_flow.jpeg}
    \caption{D1.}
    \label{fig:D1_flow}
\end{subfigure}
\caption{Comparison of repaired ISO/IEC 9798-4 Mechanism 5.2.1 two-pass mutual authentication protocol to D1. Note that ISO/IEC 9798-4:1999 Mechanism 5.2.1 uses a generic check function, with a MAC as one possible instantiation; it is represented here as a MAC.   The $\mathtt{Flow1}$ (resp. $\mathtt{Flow2}$) value corresponds to a protocol flow position indicator introduced by \cite{basin2013provably}. 
    $\mathtt{TS_S}$ (resp. $\mathtt{TS_C}$) is
    incorporated into the derivation of
    $\mathtt{K_{sc}}$ (resp. $\mathtt{K_{cs}}$).
    $\mathtt{K_{sc}}$ and $\mathtt{K_{cs}}$ also address the directional separation.
    $\mathtt{OpenFlow\_Hello}$ messages constitute the
    authenticated text $\mathtt{Text_x}$ (note that in
    ISO/IEC 9798-4:1999 Mechanism 5.2.1, it is not required that all
    text fields are the same). }
    \label{fig:9798_compare}
\end{figure}


\subsection{D3 Security}

The PEP logic requires that D1 is completed before starting D3, thereby ensuring that mutual authentication has taken place.  On the completion of D1, the switch and controller proxies create UDKs used for D3.
The security goal of D3 is to provide an authentication layer for the remainder of the controller/switch session. In this case, the authenticated ``data'' is in fact the actual OpenFlow packet. Keys for this derivative are derived as shown in Fig.~\ref{fig:keyderivation}. D3 makes use of a 512-bit MAC that allows for a longer MAC lifetime than D1. Additionally, D3 incorporates uni-directional sequence numbers into the MAC calculation step as seen in Fig.~\ref{fig:keyusage}.  Notably, this limits the potential for replay of messages by an attacker, which is of particular concern in an SDN due to the controller sending configuration commands to the switch.  If an attacker was able to replay an old configuration command, then the switch may start routing traffic improperly or the update may result in erratic network behavior.  
% Another alternative to the use of time windows is the incorporation of sequence numbers into the data sent by each side.  Upon receipt of a message, the appropriate counter is checked along with the MAC to pass the authentication check.  This allows for the elimination of the replay attack window resulting from using timestamp validity periods.


\subsection{Summary}

In this section we discussed the security goals of D1 and D3.  We made the argument that D1 provides mutual authentication between a switch and controller based on prior work on a similar ISO/IEC protocol.  We then linked D1 to D3 through the use of a session identified derived in D1 with D3's goal of providing an authentication layer for the remainder of the session.  We did not conduct a formal security proof of the composition of D1 and D3.  Instead, we leave that to future work.






 

% Protocol 3-KA-11? ISO 17770
% replace $r_a, r_b$ with implied timestamp
% text1 and text2 are the OpenFlow Hello messages
% $r^'_a$ replace with respective long-term secret key
% crunch down to two flows
% ref: Improving the ISO/IEC 11770 standard for key management techniques
% Cremers/Horvat
% Paper points out entity authentication of A to B is broken, but only because not sharing a long-term secret, which we are doing
% Also missing implicit key authentication, but should also be solved by policy engine authenticating the MAC's and we aren't sharing the key since done OOB.  So ours is more of an explicit key authentication.
% We have the assumption that the switch and controller are not compromised also
% I don't think we need any of the other security guarantees for D1.

% ISO 9798 maybe better
% rogaway and stegers without alleason 
% show key derivation process 
% discussion on correctness (derivation of key)
% discuss how works top to bottom (diagram it out)
% D1 discussion
% D3 discussion 

% IGNORE THIS SECTION FOR NOW

%The security goals of D1 and D3 are different, but they are still linked in that the completion of D1 allows for the start of D3.  

% In this sense, D1 is acting as a gatekeeper prior to the initiation of the TLS handshake.  This separation of goals allows for the security analysis of D1 to be separated from the security analysis of D3.  Any attacker who is successful at breaking the D1 verification step, will not have an advantage in the D3 step.  Instead, a successful attack on D1 would just allow for the client and server to proceed to using D3.    



% Additionally, D1 keys are ratcheted after each use in order to prevent replay attacks.  For instance, if the keys were not changed, the initial OpenFlow Hello message from either side would be the same each time the protocol was initiated.  
% In this case an attacker could attack a switch in order to force it to behaving as a normal switch and then impersonate the switch to the controller, satisfying a D1 check.  Furthermore, D3 keys are also ratcheted during the TLS handshake to prevent similar replay attacks.  After the TLS handshake is completed, TLS provides replay protection, so an additional layer of replay protection is not necessary. It is also the case that through the TLS replay protection, it is very unlikely that a message-tag pair in one session between the switch and controller will have a matching message-tag pair in another session.  Therefore, it is no longer necessary to ratchet the D3 keys and doing so would add to the complexity of implementation.
%trying to convey that TLS uses extra information like TCP sequence numbers when doing the encryption.  So for message M in session X to match message M' in session Y, they would need to be the exact same message down to the sequence number.  So ratcheting D3 to prevent this would be unnecessary?


% The D1 dialect focuses on modifying the OpenFlow Hello messages between a switch and controller.  As seen in Figure 3, the transaction ID is modified to include a MAC of the header. When the controller and switch are configured to conduct a TLS handshake, there is not a required OpenFlow Hello message prior to starting the handshake. Through the use of proxies, we can enforce that a OpenFlow Hello with the D1 modification check is conducted prior to allowing a TLS handshake with D3. This enforcement provides assurances to each side that the other is present on the network and that they are ready to perform a TLS handshake with D3 modification.

% Definition: we say that a protocol guarantees to an initiator A \emph{recent weak agreement} with another agent B if, whenever A (acting as initiator) completes a run of the protocol, apparently with responder B, then B has recently been running the protocol within authentication time $t$, apparently with A.

% Definition: MAC security from Introduction to Modern Cryptography, Phillip Rogaway and Mihir Ballare

% Definition: MAC oracle for the adversary to use??. 

% Theorem: If the controller and switch are uncompromised, then the Derivative 1 implementation provides \emph{recent weak agreement within 1 second} of the controller and switch.

% Proof: In order to break the weak agreement of the switch and controller, an attacker needs to successfully forge a message from either side. Thus the advantage of Adversary A in attacking recent weak agreement is less than or equal to the advantage in attacking the MAC security of D1.  The D1 implementation utilizes a 32-bit MAC constructed using the Blake2B protocol, which is itself collision resistant up to 256-bits. The bit strength of a 32-bit mac against collisions is $2^16$, which results in a MAC life of about 6 seconds, the average time it will take an attacker to find a collision based on parameters X,Y,Z.
% The D1 implementation, however, uses a one-time key during the MAC calculation due to the salting of the key with the current epoch time. Additionally, through the use of proxies to perform the D1 verification, we can easily restrict an attacker to X attempts to conduct a forgery of a D1 message.  Therefore, the probability of an attacker successfully forging a D1 message is negligible.


% The D3 dialect initially focuses on the additional protection of the TLS handshake. At this point of the control plane setup, D3 is designed to provide additional protection to the TLS handshake to prevent cipher suite attacks. After completion of the handshake, as seen in figure 3, the D3 dialect provides a 512-bit MAC to the TLS protected OpenFlow data. At this point, the dialect is providing an additional layer of security to the security already provided by TLS.  Thus D3 does not need to provide complete security to the messages and can be modified based on the implementer's need.

% Theorem: The composition of the Derivative 3 implementation with TLS provides MAC security within 1 second during the handshake.

% Proof: Same idea that since D3 uses keys valid for a 1 second interval during the handshake, the probability that an attacker can successfully forge a message with 512-bit MAC is negligible.  Additionally, downgrade attacks are message specific and only happen at the beginning of the handshake, so the contents of the forgery are also important as opposed to allowing acceptance of any message to break the MAC security??


% The MAC calculation/verification process for the switch is shown below.  The process is similar for the controller.

% (D1)

% MAC\_CALC($M_{sc})=$MAC($M_{sc}$, HKDF($K^1_{sc}$, freshness value))

% MAC\_VERIFY($M_{cs})=$MAC($M_{cs}$, HKDF($K^1_{cs}$, freshness value))

% (Session ID)

% SESSION\_ID=MAC\_CALC($M_{sc}$)|MAC\_VERIFY($M_{cs}$)


% (D3)

% MAC\_CALC($M_{sc})=$MAC($M_{sc}$, HKDF($K^3_{sc}$, freshness value), session ID)

% MAC\_VERIFY($M_{cs})=$MAC($M_{cs}$, HKDF($K^3_{cs}$, freshness value), session ID)

% IGNORE THIS SECTION FOR NOW

==> Prior_to_Swap_files/evaluation.tex <==
\section{Experimental Evaluation}
\label{sec:evaluation}

In this section we present results from our experimentation with the D1 and D3 derivatives in a tested built with the Mininet SDN emulation software~\cite{mininet}. 
%All experimental steps performed included: baseline testing, PEP design and testing outside of Mininet, implementation of D1, D2 and D3 with Mininet, and testing of those same derivatives to stop a cipher suite downgrade attack. 
The testbed topology with the PEPs is shown in Fig.~\ref{fig:Mininet_Experiment_Topology}. The raw packet data as well as timing statistics were captured using the Wireshark tool~\cite{wireshark}.  



\begin{figure}[ht]
    \centering
    \includegraphics[width=87mm]{figs/experiment_topology.jpeg}
    \caption{Mininet Testbed Typology}
    \label{fig:Mininet_Experiment_Topology}
\end{figure}

%We performed an experiment to assess the ability of the proxy to detect and stop a cipher suite downgrade attack performed in the untrusted medium by a man-in-the-middle.

\subsection{Mitigation of Cipher Suite Downgrade Attacks}

The first experiment that we performed was a validation to ensure the derivatives can defend against some cipher-suite downgrade attacks. 
%Once the first dialect proxy has made its modifications, 
We assume that an attacker can modify packets at will between the controller and the switch. Therefore, it is the responsibility of the receiving proxy to enforce that the modified packet by the attacker does not make it to the end point device. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=87mm]{figs/Dialect_Downgrade_Attack.jpeg}
    \caption{Timing Diagram of Downgrade Attack Experiment. The initial Hello messages exchanged by the proxies are OpenFlow Hello messages.  D1\_MAC / D3\_MAC corresponds to the MAC performed during that derivative as seen in Fig.~\ref{fig:keyusage}.}
    \label{fig:downgrade_dialect_exp}
\end{figure}


The attack method for the experiment is shown in  Fig.~\ref{fig:downgrade_dialect_exp}. In this experiment we modified the data in the first message of the TLS handshake (i.e., the switch's Client Hello) from TLS version 1.2 to 1.0 before the message was delivered to the PEP for the controller. Two versions of the attack were carried out, corresponding to the two cases where the attack message carried a D3 MAC computed by the switch's PEP and one using a wrongly guessed key.  In both cases, the receiving PEP successfully rejected the attack packet by flagging the wrong D3 MAC value.
%or indicating violation of the pre-specified security policy against advertising an outdated TLS version.  %Once the controller proxy received the message it parsed out the MAC and checked the TLS message for integrity. Upon identifying the malicious packet, it did not allow it to pass to the controller.
Consequently, the PEP sent an alert to the controller so that the controller could terminate the TLS handshake.

We note that it is straightforward to add logic to the PEPs to ensure that the cipher suite advertised by each party conforms to the IETF guidelines~\cite{rfc7507,rfc7525}. For brevity, we omit such experiments.  
%Instead, the proxy sent a known packet to the controller that is treated as an OpenFlow protocol failure and therefore terminates the connection.


%Two different attacks are available in our open-source proxy experiment. The first attack example utilized a modified Client Hello packet by replacing content in the message. The second method of attack that we performed was creating a new malicious packet and MAC, which was also denied by the PEP because the attacker did not know the key used to create the MAC. 

\subsection{Estimation of Communication Overhead}

After verifying that the proxies could be used to stop a TLS downgrade attack, we conducted a series of experiments to quantify the communication overhead from using the D1 and D3 derivatives.  
Baseline experiments without utilizing the PEPs were performed, and to examine the impact of TLS on communication latency, some experiments were also conducted without turning on TLS. 
%This baseline data was used for comparison once D1 and D3 were added to determine a percent overhead increase. The additional overhead was used to determine if D1 and D3 would meet the organization's requirements for availability due to the added security.
Specifically, we conducted a total of 90 tests for three different types of experiments as summarized in Table~\ref{table:experiment_runs}.

\begin{table}[htbp]
\caption{Summary of Overhead Measurement Tests}
\begin{center}
\begin{tabular}{|l|l|}
\hline
\textit{\textbf{Experiment Type}} & \textit{\textbf{Number of Runs}} \\ \hline
Baseline & 30 \\ \hline
TLS Enabled & 30 \\ \hline
% TLS Disabled and D1/D2 Enabled & 30 \\ \hline
TLS Enabled and Using D1 \& D3 & 30 \\ \hline
\end{tabular}
\label{table:experiment_runs}
\end{center}
\end{table}


By default, TLS is disabled in Mininet which allows for the observation of traffic and the protocol. Therefore, we performed timing first without the PEPs added to the system. The average time to establish a connection between a controller and switch was measured to be 5 seconds. To perform control testing with TLS required a generic setup and the establishment of certificates~\cite{ggee_2014}. Enabling TLS with Wireshark also requires the use of the preinstalled ovs-testcontroller as well as an OVSSwitch. The average time to establish a connection with TLS was measured to be 9.33 seconds. 


In the next step of the experiment, 
%we created the proxies in Python based on the protocol dialect creation process shown in Fig.~\ref{fig:method}. 
delays with and without TLS were measured from the first OpenFlow Hello to the first OpenFlow Echo Request message. This measurement was taken because it demonstrates the complete process to setup a new connection between the switch and controller. The OpenFlow Echo Request message signifies that all setup actions have completed and the devices are switching to a liveliness check state~\cite{of1.5}. 



% The overhead increase due to the addition of D1 and D2 was less than 1\%. 
A summary of the average connection time measurements and the average percentages of latency increase due to TLS and the derivatives are shown in Table~\ref{table:exp_results}. The overhead added by the derivatives without using TLS was minimal. Using TLS alone significantly increased the connection latency, by an average of about 186\%.  Then, deploying the derivatives on top of TLS further increased the latency by  an average of approximately 22\%. This larger overhead increase (compared to the the case without using TLS) can be attributed to the increased number of packets transmitted with D3 checks and the larger packet sizes of TLS. Still, we consider the connection latency increase over TLS to be moderate, unlikely to impact network availability.


\begin{table}[htbp]
\caption{Summary of Average Connection Latency}
\resizebox{87mm}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{TLS Enabled} & \textbf{Using D1 \& D3} & \textbf{Average Latency} & \textbf{Overhead Added} \\ \hline
No & No & 5.00 Seconds & N/A \\ \hline
No & Yes & 5.0071 Seconds & 0.041\% \\ \hline 
Yes & No & 9.33 Seconds & 186\% \\ \hline
Yes & Yes & 11.37 Seconds & 21.86\% \\ \hline
\end{tabular}%
}
\label{table:exp_results}
\end{table}


The virtual machine, scripts, packages, and Mininet used to perform this experiment are available freely and are open-source.\footnote{https://tinyurl.com/teqedac} The virtual machine provided contains bash scripts to perform the all the experiments described in this section.
%with and without TLS and with/without the derivatives described in this paper. 
The administrator account password is set to "default" for modification and running all experiments. Running the above experiments only requires commands in a command line interface. 



 




==> Prior_to_Swap_files/method_end.tex <==
\subsection{Dialect Design}

%Geoff: Explain why we design three derivatives
% Also, the use of pre-shared (salts) keys along with clock synchronization requirement at controller and each switch and the selection of different replay protection primitives.

The choices made in the dialect design stage will affect all future stages.  For this reason, it is important to consider how the choices made will impact key stages such as security and implementation, and revisit design choices during those stages.  Derivative design choices important to this stage include a protocol, algorithm class, algorithm, and key generation and management. From the protocol analysis stage, we initially identified three possible derivatives that allowed for various security goals and levels of modification within the OpenFlow protocol.  Derivative 1 (D1) modifies data within the bounds of the protocol, but utilizes a field with a small size, requiring special consideration to limit against potential forgeries. Derivative 2 (D2) relies upon a large customizable message type to add security; however, it is more readily apparent to an observer if TLS is not enabled. Lastly, D3 is the most obvious to an attacker because it modifies the contents of every packet of data sent between devices, but is removed before being processed by the endpoint.  A more detailed explanation of each derivative follows.

{\bf Derivative 1 Design}. The first potential option we identified is located in the OpenFlow header with its role in starting controller and switch communication.  The OpenFlow header is shown in Fig.~\ref{fig:derivative_overview} and is used across all message types for the OpenFlow protocol.  The 32-bit transaction ID field of the header is normally random, and is the largest field. This field is the optimal choice for the implementation of D1 since modifications to it could add security while remaining in the bounds of the protocol specification. The first message between a controller and switch is the OpenFlow Hello type message and it only consists of the OpenFlow header~\cite{of1.5}. This presents an opportunity to add security to OpenFlow starting with the very first message.

{\bf Derivative 2 Design}. The second option that we identified was derivative 2 (D2). D2 utilizes the OpenFlow Experimenter type message, which allows for a variable length data field without the previous restrictions of 32-bits for the transaction ID field from the OpenFlow header~\cite{of1.5}. The variable length field of this experiment message allows for functionality such as verification tags of other messages, key exchange data, adding sequence numbering, and dialect management. This variability allowed us to design a message type to incorporate a digest for added integrity. The message format designed for D2, with a TLS wrapper, is shown in Fig.~\ref{fig:derivative_overview}.

{\bf Derivative 3 Design}. The third option we identified and included in our experiment was a wrapper, derivative 3 (D3). Since each proxy is colocated with a device, we identified one method to not modify or require knowledge of the protocol contents. In this derivative, a MAC tag is appended to encrypted data before sending data across the untrusted communication path. This MAC tag is also removed before being passed to the attached endpoint to ensure that the OpenFlow data itself still meets the requirements of the OpenFlow standard. This MAC tag provides another way, besides TLS, to verify that no modification has occurred while traversing the untrusted medium. This option is flexible in design, length, and use because the protocol is not negatively effected and the size of a tag can be the size that an organization requires for additional security.

For this paper, we decided to focus on utilizing D1 and D3 and defer a detailed investigation of D2 use cases to future work.  A summary of the options selected for D1 and D3 are shown in Table~\ref{table:security_selections}. 


\begin{table}[htbp]
\caption{Derivative D1 \& D3 Security Selections}
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
\textit{\textbf{Derivative Security Options}} & \multicolumn{2}{l|}{\textit{\textbf{Selected Options}}} \\ \hline
Information Security Objective & \multicolumn{2}{l|}{HKDF} \\ \hline
\multicolumn{1}{|l|}{\multirow{2}{*}{Replay Protection}} & D1 & 1-Second MAC Lifetime \\ \cline{2-3} 
\multicolumn{1}{|c|}{} & D3 & Unidirectional Sequence Number \\ \hline
Algorithm & \multicolumn{2}{l|}{HMAC} \\ \hline
Sub-Algorithm & \multicolumn{2}{l|}{BLACK2b} \\ \hline
\end{tabular}%
\label{tab1}
\label{table:security_selections}
\end{center}

\end{table}




Authenticity and integrity of OpenFlow data is critical to communications between a controller and the switches it commands. Any modification of commands between the two devices can cause the failure of packet routing or unauthorized changes. Therefore, we selected HMAC as the security algorithm for D1/D3. HMAC relies upon both a secret key and the data for the commands. We selected BLAKE2b as the primary sub-algorithm to quickly create secure digests in both proxies~\cite{2013blake2}. 
To aid in the development of keys unique to each derivative, we utilize a Hash-based Key Derivation Function (HKDF).  As seen in Fig.~\ref{fig:keyderivation}, we utilize positional tagging and time based inputs to ensure keys are uni-directional as well as freshly generated when connections are initiated.  To combat replay attacks, we also incorporated mechanisms to ensure that the MAC life of all digests in the system are short.  As seen in  Table~\ref{table:security_selections}, D1 limits the MAC lifetime to 1 second.  The reason for the short lifetime is driven by the relatively short MAC values used.  D3 has a much larger MAC value, so we incorporated unidirectional sequence numbers in lieu of using timestamps for each message.



\subsection{Security and Cost Analysis}
The security and cost analysis stage is an intermediate analysis step to ensure that these objectives have been met. An organization's requirements determine if the added security is sufficient as well as the impact on overhead and system delay. The addition of security causes the use of additional processing power, memory, and time. If the self-determined criteria are not met during this intermediate analysis, then the dialect designer must return to stage 1. If the security objectives have been met, then the designer may continue in the process to determine the implementation method. 

For the sake of clarity, we defer the analysis of our design choices (which is a key part of this work) to its own section (Section~\ref{sec:analysis}).



\subsection{Implementation Method}


%There are a variety of methods to implement a protocol dialect, such as binary modification, proxies, and electromagnetic modification. Binary modification requires the direct modification of code at the device that is already installed in a system. This code modification would include the dialect, key management, and logic required to enforce the dialect.

{\bf Deployment via Policy Enforcement Proxy}. We selected proxies as our method of implementation because this system allows for rapid testing and immediate feedback during testing. For the remainder of this paper we will use the terms policy enforcement proxy (PEP) and proxy interchangeably. An example of the proxy system implementation method is shown in Fig.~\ref{fig:proxymethod} and expanded in Fig.~\ref{fig:Security_enforcement_design}. This method of implementation provides a packet by packet inspection and modification capability. 

\begin{figure}[htbp]
    \centering
    \includegraphics[width=90mm]{figs/proxymethod.jpeg}
    \caption{Proxy Implementation Method.}
    \label{fig:proxymethod}
\end{figure}

The proxy system performs a variety of operations to support normal OpenFlow operations and security mechanisms. Those operations include the establishment of TCP/IP connections with its respective device and proxy, key management/generation, dialect creation, dialect verification, and data forwarding. The components of our designed PEP are summarized and shown in Fig.~\ref{fig:Security_enforcement_design}. We expect that the PEPs can enforce and regulate other protocols and features besides OpenFlow and TLS as discussed in Section~\ref{sec:discussion}.


\begin{figure}[ht]
    \centering
    \includegraphics[width=85mm]{figs/ProxyServerLayout.jpeg}
    \caption{Policy Enforcement Proxy Design. This figure demonstrates the logical setup of the proxy and how data is managed between functions.}
    \label{fig:Security_enforcement_design}
\end{figure}


A pseudo code overview for the logic in the controller proxy is provided next. This overview provides for TCP connections between the proxies and their associated devices. Limitations associated with this generic conversation style are described in Section~\ref{sec:discussion}. Note that the derivative functions are not defined here. All scripts are available and provided at the end of this section.  

{\footnotesize
\begin{verbatim}
   
    controller_sock = make_socket
    controller_sock.connect
    proxy_to_proxy_sock = make_socket
    proxy_to_proxy_sock.listen(1)
   
    ikm = hmac_sha512(KEY_OOB, SALT)
    salt = get_salt()
    key = hkdf(ikm)
   
    data = proxy_connection.recv
    receipt = D1_check(receipt, ikm, salt)
    if(receipt == PASS):
      D1_pass = True
    else:
      D1_pass = False
    
    while(true):
        data = proxy_connection.recv
        receipt = D3_check(receipt, ikm, salt)
        if(receipt == PASS):
            controller_sock.sendall(receipt)
        else:
            controller_sock.sendall(FAIL_MSG)

        data = controller_sock.recv()
        receipt = D3_create(receipt, ikm, salt)
        proxy_connection.sendall(receipt)
        
\end{verbatim}
}


\subsection{Dialect Management}
%Dialect management design follows the selection of an implementation method. 
This stage involves the support systems and methods that will allow for PEPs to operate long-term and in day-to-day operations. Attributes important to dialect management include ease of management, installation difficulty, and scalability. 

To maximize security, our design of OpenFlow derivatives should require an independent key management system. Conceivably, to reduce the deployment cost, the operator may choose to reuse the same physical infrastructure for distributing TLS keys. In such a scenario, we recommend to use virtualization techniques to establish a logical partition between critical computing, storage, and communication resources used for the two key distribution requirements. We envision the D2 derivative to provide a communication mechanism for the controller to deliver new D1/D3 keys as well software updates to the proxies. 
% Important design factors to consider when determining a dialect management support system is the difficulty of installation, upkeep, and scalability. 

\begin{comment}

As mentioned in the implementation method stage, the selected method will require time to enforce and add to the system. While binary may be the longest to install, it provides less risk of circumventing proxy and device communication. In comparison, the selection of a proxy implementation method provides rapid addition of a dialect into an existing system. 

Dialect management includes the consideration of day-to-day and circumstantial dialect modification. Key management is at the discretion of the designer, but the dialecting proxies and D2 provide a means of updating keys and other proxy actions. In the event of resetting a PEP, enabling defense, and performing software updates this could be performed through D2 or other dialect management tools.  
\end{comment}

\subsection{Implementation Testing}
Implementation is the last stage of our protocol dialect process. Implementation testing consists of confirming security properties and identifying the availability of the system or protocol with the included dialect. Before this testing can occur, control tests of normal operation are performed and later used for comparison following dialect integration. The communication latency and other types of overhead added due to the addition of a dialect are then measured and calculated to ensure that availability of the system meets an organization's requirements. Again for clarity of presentation, we defer the details of our testing efforts to Section~\ref{sec:evaluation}.
